Introduction to Presentation Attack Detection in Iris Biometrics and Recent Advances

Iris recognition technology has attracted an increasing interest in the last decades in which we have witnessed a migration from research laboratories to real world applications. The deployment of this technology raises questions about the main vulnerabilities and security threats related to these systems. Among these threats presentation attacks stand out as some of the most relevant and studied. Presentation attacks can be defined as presentation of human characteristics or artifacts directly to the capture device of a biometric system trying to interfere its normal operation. In the case of the iris, these attacks include the use of real irises as well as artifacts with different level of sophistication such as photographs or videos. This chapter introduces iris Presentation Attack Detection (PAD) methods that have been developed to reduce the risk posed by presentation attacks. First, we summarise the most popular types of attacks including the main challenges to address. Secondly, we present a taxonomy of Presentation Attack Detection methods as a brief introduction to this very active research area. Finally, we discuss the integration of these methods into Iris Recognition Systems according to the most important scenarios of practical application.

==> Makefile <==
# Created by Sebastien Marcel <marcel@idiap.ch> 
# Wed 12 Apr 15:18:46 CEST 2017

# Builds the LaTeX project as a PDF document

TEXFILE=author.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex 
	latex $(@:%.pdf=%.tex)
	makeindex -s svind.ist author.idx
	makeindex -t author.glg -o author.gls -s myglo.ist author.glo
	@if [ -e references.bib ]; then \
	 bibtex $(@:%.pdf=%); \
	 latex $(@:%.pdf=%); \
	fi
	latex $(@:%.pdf=%.tex)
	dvipdf author

all: $(PDFFILE)

.PHONY: clean 

clean:
	@rm -vf $(shell find . -name "*~")
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.bbl *.blg
	@rm -vf *.aux *.glo *.gls *.glg *.dvi *.ps *.pdf *.out *.brf

